QUADS: QUAntized Distillation Framework for Efficient Speech Language Understanding

Spoken Language Understanding (SLU) systems must balance performance and efficiency, particularly in resource-constrained environments. Existing methods apply distillation and quantization separately, leading to suboptimal compression as distillation ignores quantization constraints. We propose QUADS, a unified framework that optimizes both through multi-stage training with a pre-tuned model, enhancing adaptability to low-bit regimes while maintaining accuracy. QUADS achieves 71.13\% accuracy on SLURP and 99.20\% on FSC, with only minor degradations of up to 5.56\% compared to state-of-the-art models. Additionally, it reduces computational complexity by 60--73$\times$ (GMACs) and model size by 83--700$\times$, demonstrating strong robustness under extreme quantization. These results establish QUADS as a highly efficient solution for real-world, resource-constrained SLU applications.

==> table/00_slurp_main_result.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
% \usepackage[normalem]{ulem}
% \useunder{\uline}{\ul}{}
% \begin{table}[]
\caption{Table Caption}
\resizebox{0.99\textwidth}{!}{
\begin{tabular}{l|rrrrrr}
\hline
Baseline                                                              & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Bit\\Length\end{tabular}} & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}\#Param\\(M) $\downarrow$\end{tabular}} & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Model\\Size (MB) $\downarrow$\end{tabular}} & \multicolumn{1}{c}{GMACs $\downarrow$}           & \multicolumn{1}{c}{Accuracy $\uparrow$} & \multicolumn{1}{c}{F1-Score $\uparrow$} \\ \hline
CTL            & 32                             & 127.00                          & 484.47                              & 143.20 & 90.14                        & 82.27                        \\
CTL                                           & 32                             & 127.00                          & 484.47                              & 143.20                              & 72.56                        & 43.34                        \\
Whisper (base)                                                        & 32                             & 20.00                           & 75.73                               & 43.72                               & 71.70                        & 65.48                        \\
Prosody                                                               & 32                             & 21.04                           & 80.27                               & 43.82                               & 68.23                        & 62.55                        \\
\begin{tabular}[l]{@{}l@{}}Prosody + \\ Distillation\end{tabular}                                                & 32                             & 21.47                           & 81.92                               & 44.09                               & 76.26                        & 71.92                        \\ \hline
\rowcolor[HTML]{E7FAE6} 
\cellcolor[HTML]{E7FAE6}{\color[HTML]{333333} }                       & {\color[HTML]{333333} 32}      & {\color[HTML]{333333} \textbf{7.85}}     & {\color[HTML]{333333} 27.66}        & {\color[HTML]{333333} \textbf{15.60}}        & {\color[HTML]{333333} 66.79} & {\color[HTML]{333333} 62.27} \\
\rowcolor[HTML]{E7FAE6} 
\cellcolor[HTML]{E7FAE6}{\color[HTML]{333333} }                       & {\color[HTML]{333333} 16}      & {\color[HTML]{333333} \textbf{7.85}}     & {\color[HTML]{333333} 13.83}        & {\color[HTML]{333333} \textbf{15.60}}        & {\color[HTML]{333333} 65.47} & {\color[HTML]{333333} 61.81} \\
\rowcolor[HTML]{E7FAE6} 
\cellcolor[HTML]{E7FAE6}{\color[HTML]{333333} }                       & {\color[HTML]{333333} 8}       & {\color[HTML]{333333} \textbf{7.85}}     & {\color[HTML]{333333} 6.91}         & {\color[HTML]{333333} \textbf{15.60}}        & {\color[HTML]{333333} 64.91} & {\color[HTML]{333333} 60.89} \\
\rowcolor[HTML]{E7FAE6} 
\multirow{-4}{*}{\cellcolor[HTML]{E7FAE6}{\color[HTML]{333333} \ourapproach}}                       & {\color[HTML]{333333} 4}       & {\color[HTML]{333333} \textbf{7.85}}     & {\color[HTML]{333333} \textbf{3.46}}         & {\color[HTML]{333333} \textbf{15.60}}        & {\color[HTML]{333333} 64.12} & {\color[HTML]{333333} 59.78}  \\ \hline
% \rowcolor[HTML]{E7FAE6} 
% \multirow{-5}{*}{\cellcolor[HTML]{E7FAE6}{\color[HTML]{333333} Ours}} & {\color[HTML]{333333} 2}       & {\color[HTML]{333333} \textbf{7.85}}     & {\color[HTML]{333333} 1.73}         & {\color[HTML]{333333} \textbf{15.60}}        & {\color[HTML]{333333} 59.15} & {\color[HTML]{333333} 58.71} \\ \hline
\end{tabular}
}

% \end{table}
